G4CASCADE: A data-driven implementation of (n, $\gamma$) cascades in Geant4

De-excitation $\gamma$ cascades from neutron captures form a dominant background to MeV-scale signals. The Geant4 Monte Carlo simulation toolkit is widely used to model backgrounds in nuclear and particle physics experiments. While its current modules for simulating (n, $\gamma$) signals, G4NDL and G4PhotoEvaporation, are excellent for many applications, they do not reproduce known gamma-ray lines and correlations relevant at 2-15 MeV. G4CASCADE is a new data-driven Geant4 module that simulates (n, $\gamma$) de-excitation pathways, with options for how to handle shortcomings in nuclear data. Benchmark comparisons to measured gamma-ray lines and level structures in the ENSDF database show significant improvements, with decreased residuals and full energy conservation. This manuscript describes the underlying calculations performed by G4CASCADE, its various usage options, and benchmark comparisons. G4CASCADE for Geant4-10 is available on GitHub at https://github.com/UCRDarkMatter/CASCADE

==> authors_svjour.tex <==
\author{\mbox{Leo Weimer}\thanksref{eleo,UCR,WVU}
        \and
        \mbox{Michela Lai}\thanksref{emichela,UCR} %etc.
        \and 
        \mbox{Emma Ellingwood}\thanksref{eemma,Queens}
        \and 
        \mbox{Shawn Westerdale}\thanksref{eshawn,UCR}
}

\thankstext{eleo}{e-mail: ljw00010@mix.wvu.edu}
\thankstext{emichela}{e-mail: michela.lai@ucr.edu}
\thankstext{eemma}{e-mail: emma.ellingwood@queensu.ca}
\thankstext{eshawn}{e-mail: shawn.westerdale@ucr.edu}
\institute{Department of Physics and Astronomy, University of California, Riverside, CA 92521, USA \label{UCR}
           \and
           Department of Physics and Astronomy, West Virginia University, Morgantown, WV 26506, USA \label{WVU}
           \and
           Department of Physics, Engineering Physics and Astronomy, Queen’s University, Kingston, ON K7L 3N6, Canada\label{Queens}
}

